Interference Alignment in MIMO Interference Channels using SDP Relaxation

Nowadays, providing higher data rate is a momentous goal for wireless communications systems. Interference is one of the important obstacles to reach this purpose. Interference alignment is a management technique that align interference from other transmitters in the least possible dimension subspace at each receiver and as a result, provide the remaining dimensions for free interference signal. An uncoordinated interference is an example of interference which cannot be aligned coordinately with interference from coordinated part and consequently, the performance of interference alignment approaches is degraded. In this paper, we propose two rank minimization methods to enhance the performance of interference alignment in the presence of uncoordinated interference sources. Firstly, a new objective function is chosen then, a new class of convex relaxation is proposed with respect to the uncoordinated interference which leads to decrease the optimal value of our optimization problem. Moreover, we use schatten-p-norm as surrogate of rank function and we implement iteratively reweighted algorithm to solve optimization problem. In addition, we apply our proposed methods to mitigate interference in relay-aided MIMO interference channel, and propose a weighted-sum method to improve the performance of interference alignment in the amplify-and-forward relay-aided MIMO system based on the rank minimization approach. Finally, our simulation results show that our proposed methods can obtain considerably higher multiplexing gain and sum rate than other approaches in the interference alignment framework and the performance of interference alignment is improved.

==> References.tex <==
	
	@article{cadambe2008interference,
		title={Interference alignment and degrees of freedom of the-user interference channel},
		author={Cadambe, Viveck R and Jafar, Syed Ali},
		journal={Information Theory, IEEE Transactions on},
		volume={54},
		number={8},
		pages={3425--3441},
		year={2008},
		publisher={IEEE}
	}
	@ARTICLE{Kim2005, 
		author={I. Y Kim and O. L. De weck}, 
		journal={Structural and Multidisciplinary Optimization}, 
		title={Adaptive weighted-sum method for bi-objective optimization: pareto front generation}, 
		year={2005}, 
		volume={29}, 
		number={2}, 
		pages={631-657}
	}
	
	@ARTICLE{Das1998, 
		author={I. Das and J. E. Dennis}, 
		journal={SIAM journal on optimization}, 
		title={NORMAL-BOUNDARY INTERSECTION: a new method for
			generating the pareto surface in nonlinear
			multicriteria optimization problems}, 
		year={1998}, 
		volume={8}, 
		number={3}, 
		pages={631-657},  
		month={Aug}
	}
	
	@Book{Bert2011, 
		author={D. P. Bertsekas}, 
		publisher={Singapore. Athena Scientific}, 
		title={Nonlinear Programming}, 
		year={1999}  
	}
	
	@article{ge2011note,
		title={A note on the complexity of L p minimization},
		author={Ge, Dongdong and Jiang, Xiaoye and Ye, Yinyu},
		journal={Mathematical programming},
		volume={129},
		number={2},
		pages={285--299},
		year={2011},
		publisher={Springer}
	}
	
	@article{chen2014interference,
		title={Interference alignment in dual-hop MIMO interference channel},
		author={Chen, Xiang and Song, SH and Letaief, Khaled},
		journal={Wireless Communications, IEEE Transactions on},
		volume={13},
		number={3},
		pages={1274--1283},
		year={2014},
		publisher={IEEE}
	}
	
	@article{gokul2015,
		title={Linear Beamformer Design for Interference Alignment via Rank Minimization},
		author={Sridharan, Gokul and Yu, Wei},
		journal={Signal Processing, IEEE Transactions on},
		volume={63},
		number={22},
		pages={5910--5923},
		year={2015},
		publisher={IEEE}
	}
	
	@article{zhang2015,
		title={Interference Neutralization for Non-Regenerative	Two-Way Relaying Networks—Part II: Optimization},
		author={Zhang, Jianshu and Ming Ho, Zuleita and A. Jorswieck, Eduard and Haardt, Martin},
		journal={Signal Processing, IEEE Transactions on},
		volume={63},
		number={17},
		pages={4557--4571},
		year={2015},
		publisher={IEEE}
	}
	
	@article{shi2011, 
		author={Q. Shi and M. Razaviyayn and Z. Luo and C.He}, 
		journal={IEEE Transactions on Signal Processing}, 
		title={An Iteratively Weighted MMSE Approach to Distributed Sum-Utility Maximization for a MIMO Interfering Broadcast Channel }, 
		year={2011}, 
		volume={59}, 
		number={9}, 
		pages={4331-4340}, 
		month={Sep}
	}
	
	@article{Troung2013, 
		author={K. T. Truong and P. Sartori and R. W. Heath}, 
		journal={IEEE Transactions on Signal Processing}, 
		title={Cooperative Algorithms for MIMO Amplify-and-Forward Relay Networks}, 
		year={2013}, 
		volume={61}, 
		number={5}, 
		pages={1272-1287}, 
		month={March}
	}
	
	@article{bresler2014feasibility,
		title={Feasibility of interference alignment for the MIMO interference channel},
		author={Bresler, Guy and Cartwright, Dustin and Tse, David},
		journal={Information Theory, IEEE Transactions on},
		volume={60},
		number={9},
		pages={5573--5586},
		year={2014},
		publisher={IEEE}
	}
	@article{papailiopoulos2012interference,
		title={Interference alignment as a rank constrained rank minimization},
		author={Papailiopoulos, Dimitris S and Dimakis, Alexandros G},
		journal={Signal Processing, IEEE Transactions on},
		volume={60},
		number={8},
		pages={4278--4288},
		year={2012},
		publisher={IEEE}
	}
	@article{du2013reweighted,
		title={Reweighted nuclear norm approach for interference alignment},
		author={Du, Huiqin and Ratnarajah, Tharm and Sellathurai, Mathini and Papadias, Constantinos B},
		journal={Communications, IEEE Transactions on},
		volume={61},
		number={9},
		pages={3754--3765},
		year={2013},
		publisher={IEEE}
	}
	@article{peters2011cooperative,
		title={Cooperative algorithms for {MIMO} interference channels},
		author={Peters, Steven W and Heath Jr, Robert W},
		journal={Vehicular Technology, IEEE Transactions on},
		volume={60},
		number={1},
		pages={206--218},
		year={2011},
		publisher={IEEE}
	}
	@article{damnjanovic2011survey,
		title={A survey on {3GPP} heterogeneous networks},
		author={Damnjanovic, Aleksandar and Montojo, Juan and Wei, Yongbin and Ji, Tingfang and Luo, Tao and Vajapeyam, Madhavan and Yoo, Taesang and Song, Osok and Malladi, Durga},
		journal={Wireless Communications, IEEE},
		volume={18},
		number={3},
		pages={10--21},
		year={2011},
		publisher={IEEE}
	}
	@article{ruan2013feasibility,
		title={The feasibility conditions for interference alignment in {MIMO} networks},
		author={Ruan, Liangzhong and Lau, Vincent KN and Win, Moe Z},
		journal={Signal Processing, IEEE Transactions on},
		volume={61},
		number={8},
		pages={2066--2077},
		year={2013},
		publisher={IEEE}
	}
	@article{yetis2010feasibility,
		title={On feasibility of interference alignment in {MIMO} interference networks},
		author={Yetis, Cenk M and Gou, Tiangao and Jafar, Syed A and Kayran, Ahmet H},
		journal={Signal Processing, IEEE Transactions on},
		volume={58},
		number={9},
		pages={4771--4782},
		year={2010},
		publisher={IEEE}
	}
	@phdthesis{fazel2002matrix,
		title={Matrix rank minimization with applications},
		author={Fazel, Maryam},
		year={2002},
		school={PhD thesis, Stanford University}
	}
	@book{boyd2004convex,
		title={Convex optimization},
		author={Boyd, Stephen and Vandenberghe, Lieven},
		year={2004},
		publisher={Cambridge university press}
	}
	@inproceedings{peters2009interference,
		title={Interference alignment via alternating minimization},
		author={Peters, Steven W and Heath Jr, Robert W},
		booktitle={Acoustics, Speech and Signal Processing, 2009. ICASSP 2009. IEEE International Conference on},
		pages={2445--2448},
		year={2009},
		organization={IEEE}
	}
	@article{berger2009, 
		author={S. Berger and M. Kuhn and A. Wittneben and T. Unger and A. Klein}, 
		journal={IEEE Communications Maggazine}, 
		title={Recent Advances in Amplify-and-Forward Two-hop Relaying }, 
		year={2009}, 
		volume={47}, 
		number={7}, 
		pages={50-56}, 
		month={July}
	}
	@ARTICLE{Gomadam2011Distributed, 
		author={K. Gomadam and V. R. Cadambe and S. A. Jafar}, 
		journal={IEEE Transactions on Information Theory}, 
		title={A Distributed Numerical Approach to Interference Alignment and Applications to Wireless Interference Networks}, 
		year={2011}, 
		volume={57}, 
		number={6}, 
		pages={3309-3322}
	}
	
	%@inproceedings{gomadam2008approaching,
	%	title={Approaching the capacity of wireless networks through distributed interference alignment},
	%	author={Gomadam, Krishna and Cadambe, Viveck R and Jafar, Syed A},
	%	booktitle={Global Telecommunications Conference, 2008. IEEE GLOBECOM 2008. IEEE},
	%	pages={1--6},
	%	year={2008},
	%	organization={IEEE}
	%}
	
	@inproceedings{ji2013beyond,
		title={Beyond convex relaxation: A polynomial-time non-convex optimization approach to network localization},
		author={Ji, Senshan and Sze, Kam-Fung and Zhou, Zirui and So, Anthony Man-Cho and Ye, Yinyu},
		booktitle={INFOCOM, 2013 Proceedings IEEE},
		pages={2499--2507},
		year={2013},
		organization={IEEE}
	}
	@article{mohan2012iterative,
		title={Iterative reweighted algorithms for matrix rank minimization},
		author={Mohan, Karthik and Fazel, Maryam},
		journal={The Journal of Machine Learning Research},
		volume={13},
		number={1},
		pages={3441--3473},
		year={2012},
		publisher={JMLR. org}
	}
	@misc{grant2008cvx,
		title={CVX: Matlab software for disciplined convex programming},
		author={Grant, Michael and Boyd, Stephen and Ye, Yinyu},
		year={2008}
	}
	%@article{ge2011note,
	%	title={A note on the complexity of L p minimization},
	%	author={Ge, Dongdong and Jiang, Xiaoye and Ye, Yinyu},
	%	journal={Mathematical programming},
	%	volume={129},
	%	number={2},
	%	pages={285--299},
	%	year={2011},
	%	publisher={Springer}
	%}
	@article{Liu2015,
		title={Interference Alignment for Partially Connected Downlink {MIMO} Heterogeneous Networks},
		author={Liu, Guoqing and Sheng, Ming and Wang, Xijun and Jiao, Wanguo and Li, Ying and Li, Jiandong},
		journal={Communications, IEEE Transactions on},
		volume={63},
		number={2},
		pages={551--564},
		year={2015},
		publisher={IEEE}
	}
	@ARTICLE{Gou2010, 
		author={T. Gou and S. A. Jafar}, 
		journal={IEEE Transactions on Information Theory}, 
		title={Degrees of Freedom of the  K User  M $\times$ N MIMO Interference Channel}, 
		year={2010}, 
		volume={56}, 
		number={12}, 
		pages={6040-6057},  
		month={Dec}
	}

